PhysBrain 1.0 Technical Report

Vision-language-action models have advanced rapidly, but robot trajectories alone provide limited coverage for learning broad physical understanding. PhysBrain 1.0 studies a complementary route: converting large-scale human egocentric video into structured physical commonsense supervision before robot adaptation. Our data engine extracts scene elements, spatial dynamics, action execution, and depth-aware relations, then turns them into question-answer supervision for training PhysBrain VLMs. The resulting physical priors are further transferred to VLA policies through a capability-preserving and language-sensitive adaptation design. Across multimodal QA benchmarks and embodied control benchmarks, including ERQA, PhysBench, SimplerEnv-WidowX, LIBERO, and RoboCasa, PhysBrain 1.0 achieves SOTA results and shows especially strong out-of-domain performance on SimplerEnv. These results suggest that scaling physical commonsense from human interaction video can provide an effective bridge from multimodal understanding to robot action.

==> sec/test.tex <==
\begin{figure*}[!htb]
    \centering
    \includesvg[width=1.0\linewidth, inkscapelatex=false]{fig/PhysBrainVLA.svg}
    \caption{XXX.}
    \label{fig:physbrainvla}
\end{figure*}

==> tab/vlm_qa_results.tex <==
\begin{table*}[t]
  \centering
  \small
  \setlength{\tabcolsep}{4.5pt}
  \renewcommand{\arraystretch}{1.15}
  \caption{
    \textbf{Multimodal question-answering benchmark results.}
    We compare PhysBrain 1.0 models with their Qwen3-VL base models and representative multimodal baselines.
    Higher is better for all benchmarks. We highlight the best result in \textbf{bold} and the second-best result with \underline{underline}.
  }
  \begin{adjustbox}{width=\textwidth}
  \begin{tabular}{l c c c c c c c}
    \toprule
    \textbf{Model} & \textbf{ERQA} & \textbf{PhysBench} & \textbf{MME} & \textbf{MMMU} & \textbf{OCRBench} & \textbf{RealWorldQA} & \textbf{TextVQA} \\
    \midrule
    Qwen3-VL-8B (Base) & 43.0 & 48.5 & 2373.3 & 53.2 & \underline{84.4} & 69.4 & \underline{82.1} \\
    Qwen3-VL-4B (Base) & 39.8 & 45.7 & 2297.5 & 48.4 & 82.8 & \underline{70.5} & 80.1 \\
    RoboBrain2.5-8B & \underline{43.3} & \underline{49.2} & 2410.0 & \underline{54.6} & \underline{84.4} & 70.1 & 80.8 \\
    VST-7B-RL & 40.3 & 46.4 & 2036.6 & 47.9 & 82.7 & 67.3 & 81.9 \\
    MiMo-VL-7B-RL & 38.5 & 39.4 & \underline{2413.6} & 41.0 & 81.4 & 29.8 & 76.4 \\
    \textbf{PhysBrain 4B (ours)} & 41.0 & 48.1 & 2385.1 & 49.9 & 83.0 & \textbf{72.7} & 81.1 \\
    \textbf{PhysBrain 8B (ours)} & \textbf{45.5} & \textbf{50.2} & \textbf{2431.1} & \textbf{55.2} & \textbf{85.7} & 68.8 & \textbf{83.3} \\
    \bottomrule
  \end{tabular}
  \end{adjustbox}
  \label{tab:vlm_qa_results}
\end{table*}

